A Comparative Study of the Perceptual Sensitivity of Topological Visualizations to Feature Variations

Color maps are a commonly used visualization technique in which data are mapped to optical properties, e.g., color or opacity. Color maps, however, do not explicitly convey structures (e.g., positions and scale of features) within data. Topology-based visualizations reveal and explicitly communicate structures underlying data. Although we have a good understanding of what types of features are captured by topological visualizations, our understanding of people's perception of those features is not. This paper evaluates the sensitivity of topology-based isocontour, Reeb graph, and persistence diagram visualizations compared to a reference color map visualization for synthetically generated scalar fields on 2-manifold triangular meshes embedded in 3D. In particular, we built and ran a human-subject study that evaluated the perception of data features characterized by Gaussian signals and measured how effectively each visualization technique portrays variations of data features arising from the position and amplitude variation of a mixture of Gaussians. For positional feature variations, the results showed that only the Reeb graph visualization had high sensitivity. For amplitude feature variations, persistence diagrams and color maps demonstrated the highest sensitivity, whereas isocontours showed only weak sensitivity. These results take an important step toward understanding which topology-based tools are best for various data and task scenarios and their effectiveness in conveying topological variations as compared to conventional color mapping.

==> fig.vis.colormap.tex <==


\begin{figure}[!hb]
    \centering 
    \includegraphics[width=0.875\linewidth]{figures/imagesByPaul/colormapVisNew.png}
    \caption{Example color map visualizations of the rabbit and skull models. The viridis color map, which is highly effective for identifying visual features, is used~\cite{viridis_colormap}. The purple-like hue is a global minimum, $f_{min}$, and the yellowish hue is a global maximum, $f_{max}$.}
 \label{fig:colormap_example}
\end{figure}



==> fig.vis.iso.tex <==

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.875\linewidth]{figures/imagesByTushar/isocontourVis.png}
    \caption{Example isocontour visualization on the rabbit and skull models. Birth and merging of connected components as well as high and low spatial density structures are highlighted on the rabbit. The skull is visualized with a high (top) and low (bottom) number of isocontours.}
    \label{fig:isocontour_example}
\end{figure}




==> fig.vis.pd.tex <==

\begin{figure}[!ht]
    \centering %
    \includegraphics[width=0.875\linewidth]{figures/imagesByTushar/persistenceDiagramVisRevised.png}
    \caption{An example of the persistence diagram visualization applied to the rabbit (left) and skull (right) models. The blue dots denote the saddle-minimum or saddle-maximum pairs, and red dots denote the saddle-saddle pairs. High-persistence features are farther away from the diagonal, whereas low-persistence features are closer to the diagonal. Persistence diagrams can be simplified by removing critical point pairs based on their persistence, as illustrated for the skull model (right).}
 \label{fig:persistence_diagram_example}
\end{figure}

















==> fig.vis.reeb.tex <==

\begin{figure}[!hb]
    \centering
    \includegraphics[width=0.875\linewidth]{figures/imagesByPaul/reebGraphVis.png}
    \caption{An example of the Reeb graph visualization applied to the rabbit and skull. Blue spheres denote the critical point positions, and the red arcs indicate the evolution of contours between critical points. The Reeb graphs for the skull are rendered without (top) and with (bottom) pruning, guided by the persistence of critical points.}
 \label{fig:reeb_example}
\end{figure}


